Form factors for semi-leptonic $B$ decays

Semi-leptonic $B$ decays provide promising channels to test the Standard Model, search for signs of new physics, or determine fundamental parameters like CKM matrix elements. We present an update on our calculation of short distance contributions to GIM suppressed rare $B$ decays focusing in particular on $B_s\to \phi \ell^+ \ell^-$ decays. Furthermore we show first results for our calculation of $B_{(s)}\to D_{(s)}^{(*)}\ell\nu$ semi-leptonic decays involving $b\to c$ transitions. Our calculations are based on RBC-UKQCD's 2+1 flavor domain-wall fermion and Iwasaki gauge field configurations featuring three lattice spacings in the range $1.73$ GeV $\le a^{-1} \le 2.77$ GeV and pion masses down to the physical value. We calculate the form factors by simulating $b$-quarks using the relativistic heavy quark action, create light $u/d$ and $s$ quarks with standard domain-wall kernel, and use optimised M\"obius domain-wall fermions for charm quarks.

==> Proceedings_aux <==
\relax 
\global\@todotoctrue
\citation{Glashow:1970gm}
\citation{Aaij:2015oid}
\citation{Aaij:2015esa}
\citation{Aaij:2014ora}
\citation{Grinstein:1987vj,Grinstein:1990tj,Buras:1993xp,Ciuchini:1993ks,Ciuchini:1993fk,Ciuchini:1994xa}
\citation{Buras:2002tp,Gambino:2003zm,Altmannshofer:2008dz}
\citation{Grinstein:2004vb,Beylich:2011aq}
\citation{Lyon:2014hpa}
\citation{Flynn:2015ynk}
\global\@todotoctrue
\citation{Allton:2008pn,Aoki:2010dy}
\citation{Christ:2006us}
\citation{Aoki:2012xaa}
\citation{Flynn:2015ynk}
\citation{Allton:2008pn,Aoki:2010dy}
\citation{Blum:2014tka}
\citation{Allton:2008pn,Aoki:2010dy}
\citation{Blum:2014tka}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}}
\newlabel{eq:tf-2}{{1.2}{1}}
\newlabel{eq:tf-1}{{1.3}{1}}
\@writefile{toc}{\contentsline {section}{\numberline {2}Computational setup}{1}}
\newlabel{Sec.Setup}{{2}{1}}
\global\@todotoctrue
\global\@todotoctrue
\newlabel{tab:1}{{2}{2}}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Parameters of the calculation. We use ensembles generated by the RBC and UKQCD collaboration \cite  {Allton:2008pn, Aoki:2010dy} with 2+1 flavor domain-wall fermions and Iwasaki gauge actions. The domain-wall fermions are created with fifth dimension $L_s=16$ and domain-wall height $M_5=1.8$ for . Values for the inverse lattice spacing and the quark and meson masses are taken from the refined analysis \cite  {Blum:2014tka}; $am_l$ labels the mass of the light sea-quark, $am_h$ the mass of the heavy sea quark, and $am_s$ the mass of the strange quark mass. }}{2}}
\@writefile{toc}{\contentsline {section}{\numberline {3}Preliminary results}{2}}
\newlabel{Sec.Results}{{3}{2}}
\@writefile{toc}{\contentsline {section}{\numberline {4}Summary and conclusions}{2}}
\newlabel{Sec.Summary}{{4}{2}}
\bibdata{B_meson}
\bibcite{Glashow:1970gm}{{1}{}{{}}{{}}}
\bibcite{Aaij:2015oid}{{2}{}{{}}{{}}}
\bibcite{Aaij:2015esa}{{3}{}{{}}{{}}}
\bibcite{Aaij:2014ora}{{4}{}{{}}{{}}}
\bibcite{Grinstein:1987vj}{{5}{}{{}}{{}}}
\bibcite{Grinstein:1990tj}{{6}{}{{}}{{}}}
\bibcite{Buras:1993xp}{{7}{}{{}}{{}}}
\bibcite{Ciuchini:1993ks}{{8}{}{{}}{{}}}
\bibcite{Ciuchini:1993fk}{{9}{}{{}}{{}}}
\bibcite{Ciuchini:1994xa}{{10}{}{{}}{{}}}
\bibcite{Buras:2002tp}{{11}{}{{}}{{}}}
\bibcite{Gambino:2003zm}{{12}{}{{}}{{}}}
\bibcite{Altmannshofer:2008dz}{{13}{}{{}}{{}}}
\bibcite{Grinstein:2004vb}{{14}{}{{}}{{}}}
\bibcite{Beylich:2011aq}{{15}{}{{}}{{}}}
\bibcite{Lyon:2014hpa}{{16}{}{{}}{{}}}
\bibcite{Flynn:2015ynk}{{17}{}{{}}{{}}}
\bibcite{Allton:2008pn}{{18}{}{{}}{{}}}
\bibcite{Aoki:2010dy}{{19}{}{{}}{{}}}
\bibcite{Shamir:1993zy}{{20}{}{{}}{{}}}
\bibcite{Furman:1994ky}{{21}{}{{}}{{}}}
\bibcite{Christ:2006us}{{22}{}{{}}{{}}}
\bibcite{Aoki:2012xaa}{{23}{}{{}}{{}}}
\bibcite{Blum:2014tka}{{24}{}{{}}{{}}}
\bibcite{Edwards:2004sx}{{25}{}{{}}{{}}}
\bibstyle{apsrev4-1ow}
\providecommand\NAT@force@numbers{}\NAT@force@numbers
\@writefile{toc}{\contentsline {paragraph}{Acknowledgements}{3}}

